Witt vectors and $\delta$-Cartier rings

We give a universal property of the construction of the ring of $p$-typical Witt vectors of a commutative ring, endowed with Witt vectors Frobenius and Verschiebung, and generalize this construction to the derived setting. We define an $\infty$-category of $p$-typical derived $\delta$-Cartier rings and show that the derived ring of $p$-typical Witt vectors of a derived ring is naturally an object in this $\infty$-category. Moreover, we show that for any prime $p$, the formation of the derived ring of $p$-typical Witt vectors gives an equivalence between the $\infty$-category of all derived rings and the full subcategory of all derived $p$-typical $\delta$-Cartier rings consisting of $V$-complete objects.

==> hat_en.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[autostyle, english=american]{csquotes}
\MakeOuterQuote{"}

\usepackage{xcolor}
\definecolor{reference}{rgb}{0.20,0.36,0.74}
\definecolor{citation}{rgb}{0,.40,.80}
\usepackage[colorlinks,linktocpage,urlcolor=blue,linkcolor=reference,citecolor=citation]{hyperref}
%backref

\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{latexsym}
\usepackage{graphicx}
\usepackage{amscd,amsfonts,amssymb,amsmath,amsbsy,amsthm}
\usepackage[mathscr]{eucal}
\usepackage[all, 2cell]{xy}
\UseTwocells
\xyoption{2cell}{\UseTwocells}
\usepackage{verbatim}
\usepackage{enumerate}
\usepackage{tikz}
\usepackage[left=2cm, top=2cm, right=2cm, bottom=2cm]{geometry}
\usepackage{enumitem} %[wide, topsep=\parskip, itemsep=\parskip, parsep=\parskip]
% \setlength\itemindent{\labelwidth+\labelsep} \item \setlength\itemindent{\parindent}

%\usepackage{amsrefs}
\usepackage[backend=biber,style=alphabetic,firstinits=true,maxbibnames=99,maxalphanames=99]{biblatex}
\usepackage[capitalise]{cleveref}
\crefformat{equation}{(#2#1#3)}

\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.200] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\usepackage{relsize}
%\usepackage[bbgreekl]{mathbbol}
%\DeclareSymbolFontAlphabet{\mathbb}{AMSb} %to ensure that the meaning of \mathbb does not change
%\DeclareSymbolFontAlphabet{\mathbbl}{bbold}
\newcommand{\mathbbl}{}
\newcommand{\Prism}{{\mathlarger{\mathbbl{\Delta}}}}

% Bibliography spacing
\setlength{\bibitemsep}{.2\baselineskip plus .05\baselineskip minus .05\baselineskip}
\newlength{\bibparskip}\setlength{\bibparskip}{0pt}
\let\oldthebibliography\thebibliography
\renewcommand\thebibliography[1]{%
  \oldthebibliography{#1}%
  \setlength{\parskip}{\bibitemsep}%
  \setlength{\itemsep}{\bibparskip}%
}

\newcommand{\arxiv}[1]{\href{https://arxiv.org/abs/#1}{arXiv:#1}}
\newcommand{\doi}[1]{doi:\href{https://doi.org/#1}{#1}}

% For definitions
\DeclareTextFontCommand{\emdef}{\bfseries}

% Theorems

\newtheorem{thm}{Theorem}
\newtheorem*{thm*}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem*{cor*}{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem*{prop*}{Proposition}
\newtheorem{claim}[thm]{Claim}
\newtheorem{variant}[thm]{Variant}
\newtheorem{situation}[thm]{Situation}
\newtheorem{question}{thm}{Question}
\newtheorem{computation}{thr}{Computation}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{construction}[thm]{Construction}
\newtheorem{notation}[thm]{Notation}
\newtheorem{notations}[thm]{Notations}
\newtheorem{ex}[thm]{Example}
\newtheorem{exercise}[thm]{Exercise}
\newtheorem{rem}[thm]{Remark}
\newtheorem{question}[thm]{Question}
\newtheorem{prob}[thm]{Problem}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem*{conj*}{Conjecture}
\newtheorem{conv}[thm]{Conventions}
\newtheorem{warn}[thm]{Warning}
\newtheorem{assumption}[thm]{Assumption}


\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}

\definecolor{note_color}{rgb}{0.0,0.7,0.0}
\newcommand{\note}[1]{\textcolor{note_color}{#1}}

\newcommand{\clause}[1]{\noindent\underline{\textit{#1}}}

% Commands

\newcommand{\eset}{\varnothing}
\newcommand{\fcat}{\mathscr}
\newcommand{\inj}{\hookrightarrow}
\newcommand{\surj}{\twoheadrightarrow}
\newcommand{\areq}{\mathbin{{\xrightarrow{\,\sim\,}}}}
\newcommand{\aleq}{\mathbin{{\xleftarrow{\,\sim\,}}}}

%
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\lra}{\longrightarrow}
\newcommand{\lla}{\longleftarrow}

% Linear algebra
\DeclareMathOperator{\Vect}{Vect}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Sym}{Sym}
\newcommand{\Mod}{\mathrm{Mod}}
\newcommand{\LMod}{\mathrm{LMod}}
\newcommand{\RMod}{\mathrm{RMod}}
\newcommand{\GL}{{\mathrm{GL}}}
\DeclareMathOperator{\SL}{SL}
\newcommand{\gr}{{\mathrm{gr}}}
\DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\tr}{tr}

% Algebra
\DeclareMathOperator{\St}{St}
\DeclareMathOperator{\cdgAlg}{cdg-Alg}
\DeclareMathOperator{\dgAlg}{dg-Alg}
\DeclareMathOperator{\dgMod}{dg-Mod}
\DeclareMathOperator{\coMod}{coMod}
\DeclareMathOperator{\Frac}{Frac}
\DeclareMathOperator{\Prim}{Prim}
\DeclareMathOperator{\mchar}{char}
\DeclareMathOperator{\Der}{Der}

% Representation theory
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\Rep}{Rep}
\DeclareMathOperator{\Irr}{Irr}

% Complex analysis
\DeclareMathOperator*{\ord}{ord}
\DeclareMathOperator*{\Res}{Res}
\renewcommand{\Re}{\mathrm{Re}}
\renewcommand{\Im}{\mathrm{Im}}
\DeclareMathOperator{\Ln}{Ln}
\DeclareMathOperator{\Arg}{Arg}

% Topology
\DeclareMathOperator{\td}{td}
\DeclareMathOperator{\Th}{Th}
\DeclareMathOperator{\Sq}{Sq}
\newcommand{\Top}{ {\mathrm Top} }
\newcommand{\Orb}{\mathcal{O}}
\newcommand{\SOrb}{\mathcal{SO}}
\DeclareMathOperator{\Glo}{Glo}
\DeclareMathOperator{\LocSys}{LocSys}
\DeclareMathOperator{\conn}{conn}
\DeclareMathOperator{\gl}{gl}
\DeclareMathOperator{\chern}{ch}
\DeclareMathOperator{\supp}{supp}

% Differential geometry
\newcommand{\Mfld}{ {\fcat M\mathrm{fld}} }
\newcommand{\Bndl}{ {\fcat B\mathrm{ndl}} }
\DeclareMathOperator{\Emb}{Emb}

%Algebraic geometry
\DeclareMathOperator{\spec}{spec}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Spf}{Spf}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\Pic}{Pic}
\newcommand{\HS}{\mathrm{Hdg}}
\newcommand{\MHS}{\mathrm{MHdg}}
\DeclareMathOperator{\Restr}{Res}
\DeclareMathOperator{\Qcoh}{Qcoh}
\DeclareMathOperator{\Coh}{Coh}
\DeclareMathOperator{\ICoh}{ICoh}
\newcommand{\LHom}{{\mathcal Hom}}
\DeclareMathOperator{\Moduli}{Moduli}
\DeclareMathOperator{\QCoh}{QCoh}
\DeclareMathOperator{\Bl}{Bl}
\DeclareMathOperator{\Isom}{Isom}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\Perf}{Perf}
\DeclareMathOperator{\APerf}{APerf}
\newcommand{\mstack}{\mathpzc}
\DeclareMathOperator{\PStk}{{\mathscr{PS}tk}}
\DeclareMathOperator{\Stk}{{\mathscr{S}tk}}
\newcommand{\Hdg}{{\mathrm H}}
\newcommand{\dR}{{\mathrm{dR}}}
\newcommand{\crys}{{\mathrm{crys}}}
\newcommand{\perf}{{\mathrm{perf}}}
\newcommand{\fp}{{\mathrm{fp}}}
\DeclareMathOperator{\At}{At}
\DeclareMathOperator{\Bun}{Bun}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\Aff}{Aff}
\newcommand{\sm}{{\mathrm{sm}}}
\newcommand{\Ideal}{{\mathrm{Ideal}}

%Number theory
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\Nm}{Nm}
\DeclareMathOperator{\Frob}{Frob}
\DeclareMathOperator{\rad}{rad}
\DeclareMathOperator{\Spa}{Spa}
\DeclareMathOperator{\Spv}{Spv}
\DeclareMathOperator{\HRing}{HRing}
\newcommand{\et}{{\mathrm{\acute et}}}
\newcommand{\pd}{{\mathrm{pd}}}

%Category theory
\newcommand{\Type}{ {\fcat{S}} }
\newcommand{\Set}{ {\fcat{S}\mathrm{et}} }
\newcommand{\Gpd}{ {\fcat G\mathrm{pd}} }
\newcommand{\Cat}{ {\fcat C\mathrm{at}} }
\newcommand{\Grpd}{ {\fcat Grpd} }
\newcommand{\Prs}{ {\mathrm{Pr}} }
\DeclareMathOperator{\Ob}{Ob}
\DeclareMathOperator{\Ab}{Ab}
\DeclareMathOperator{\Grp}{Grp}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Tor}{Tor}
\newcommand{\HHom}{ {\fcat Hom} }
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\EEnd}{{\mathcal End}}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Map}{Map}
\DeclareMathOperator{\Fun}{Fun}
\newcommand{\Nat}{\mathrm{Nat}}
\DeclareMathOperator{\Exc}{Exc}
\DeclareMathOperator{\Homog}{Homog}
\DeclareMathOperator{\Ho}{Ho}
\DeclareMathOperator{\core}{core}
\DeclareMathOperator{\Sp}{Sp}
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\creff}{cr}
\DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\Pro}{Pro}
\DeclareMathOperator*{\colim}{colim}
\DeclareMathOperator*{\fib}{fib}
\DeclareMathOperator*{\tfib}{tfib}
\DeclareMathOperator*{\cofib}{cofib}
\DeclareMathOperator*{\coker}{coker}
\newcommand{\SSet}{ {\mathrm{SSet}} }
\DeclareMathOperator{\Mon}{Mon}
\DeclareMathOperator{\CMon}{CMon}
\DeclareMathOperator{\Alg}{Alg}
\DeclareMathOperator{\CAlg}{CAlg}
\DeclareMathOperator{\cCAlg}{cCAlg}
\DeclareMathOperator{\LAlg}{LAlg}
\newcommand{\EnAlg}[1]{\mathrm{E_{#1}Alg}}
\DeclareMathOperator{\CRing}{CRing}
\DeclareMathOperator{\Lie}{Lie}
\DeclareMathOperator{\Lan}{Lan}
\DeclareMathOperator{\Ran}{Ran}
\DeclareMathOperator{\PreSh}{PreSh}
\DeclareMathOperator{\ev}{ev}
\DeclareMathOperator{\coev}{coev}
\DeclareMathOperator{\Free}{Free}
\newcommand{\prolim}[1][]{\lim\limits_{\xleftarrow[#1]{}}}
\newcommand{\indlim}[1][]{\lim\limits_{\xrightarrow[#1]{}}}
\DeclareMathOperator{\sk}{sk}
\DeclareMathOperator{\cosk}{cosk}
\DeclareMathOperator{\Tot}{Tot}
\newcommand{\Yon}{\mathcal Y}
\DeclareMathOperator{\Tw}{Tw}
\newcommand{\exc}{{\mathrm{ex}}}
\DeclareMathOperator{\eq}{eq}
\newcommand{\kd}{{\mathrel{\rotatebox[origin=c]{180}{$!$}}}}
\DeclareMathOperator{\triv}{triv}
\DeclareMathOperator{\sd}{sd}
\DeclareMathOperator{\Comm}{Comm}
\DeclareMathOperator{\Assoc}{Assoc}
\DeclareMathOperator{\Env}{Env}
\DeclareMathOperator{\Fil}{Fil}
\DeclareMathOperator{\Id}{Id}
\newcommand{\PShv}{{\mathcal{PS}\mathrm{hv}}}
\newcommand{\Shv}{{\mathcal S\mathrm{hv}}}
\newcommand{\op}{{\mathrm{op}}}
\newcommand{\SSeq}{{\mathrm{SSeq}}}
\newcommand{\dual}{{\mathrm{dual}}}
\newcommand{\lax}{{\mathrm{lax}}}
\newcommand{\llax}{{\mathrm{l.lax}}}
\newcommand{\rlax}{{\mathrm{r.lax}}}

%Math. phys.
\DeclareMathOperator{\crit}{crit}

%Other
\DeclareMathOperator{\sign}{sign}
\mathchardef\mdef="2D
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\DeclareMathOperator{\const}{const}

